From G\"odel's Incompleteness Theorem to the completeness of bot beliefs (Extended abstract)

Hilbert and Ackermann asked for a method to consistently extend incomplete theories to complete theories. G\"odel essentially proved that any theory capable of encoding its own statements and their proofs contains statements that are true but not provable. Hilbert did not accept that G\"odel's construction answered his question, and in his late writings and lectures, G\"odel agreed that it did not, since theories can be completed incrementally, by adding axioms to prove ever more true statements, as science normally does, with completeness as the vanishing point. This pragmatic view of validity is familiar not only to scientists who conjecture test hypotheses but also to real estate agents and other dealers, who conjure claims, albeit invalid, as necessary to close a deal, confident that they will be able to conjure other claims, albeit invalid, sufficient to make the first claims valid. We study the underlying logical process and describe the trajectories leading to testable but unfalsifiable theories to which bots and other automated learners are likely to converge.

==> PICS/cmn-left.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Sep 02 17:30:15 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.63" x-max="15" y-min="-10.62" y-max="7.5" auto-bounding="true">
%<multicurve points= "(5.62,-0.62);(5.62,-0.62);(10.62,-5.62);(10.62,-5.62);(10.62,-5.62);(9.38,-5.62);
%	(9.38,-5.62);(9.38,-5.62);(10,-5.62);(10,-5.62)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(2.81,2.19)"
%	 p2= "(2.81,-0.94)"
%	 p1= "(5.94,-0.94)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(8.75,-3.75)"
%	 p2= "(8.75,-6.88)"
%	 p1= "(11.88,-6.88)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(15,7.5);(15,7.5);(15,5);(15,5);(15,5);(15,-0.63);
%	(15,-0.63);(15,-0.63);(11.25,-4.38);(11.25,-4.38)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(9.37,7.5);(9.37,7.5);(9.37,6.87);(9.37,6.87);(9.37,6.87);(9.38,5);
%	(9.38,5);(9.38,5);(5.63,1.25);(5.63,1.25)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(-0.63,7.5);(-0.63,7.5);(-0.63,6.87);(-0.63,6.87);(-0.63,6.87);(-0.62,5);
%	(-0.62,5);(-0.62,5);(3.13,1.25);(3.13,1.25)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(10,-6.88);(10,-6.88);(10,-10);(10,-10);(10,-10);(10,-10.62);
%	(10,-10.62);(10,-10.62);(10,-10);(10,-10)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(15,7.5)
\psline(5.62,-0.62)
(10.62,-5.62)
(9.38,-5.62)(10,-5.62)
\rput{0}(4.38,0.62){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\rput{0}(10.32,-5.31){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\psline(15,7.5)
(15,5)
(15,-0.63)(11.25,-4.38)
\psline(9.37,7.5)
(9.37,6.87)
(9.38,5)(5.63,1.25)
\psline(-0.63,7.5)
(-0.63,6.87)
(-0.62,5)(3.13,1.25)
\psline(10,-6.88)
(10,-10)
(10,-10.62)(10,-10)
\end{pspicture}


==> PICS/cmn-right-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Mar 16 16:48:01 GMT-10:00 2023
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.63" x-max="15.63" y-min="-10.62" y-max="8.12" auto-bounding="true">
%<ellipse fill-style= "solid"
%	 stroke-width= "0.45"
%	 p3= "(9.06,2.19)"
%	 p2= "(9.06,-0.94)"
%	 p1= "(12.19,-0.94)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.45"
%	 points= "(15.62,8.12);(15.62,8.12);(15.62,7.5);(15.62,7.5);(15.62,7.5);(15.63,5.62);
%	(15.63,5.62);(15.63,5.62);(11.88,1.87);(11.88,1.87)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.45"
%	 points= "(5.62,8.12);(5.62,8.12);(5.62,7.5);(5.62,7.5);(5.62,7.5);(5.63,5.62);
%	(5.63,5.62);(5.63,5.62);(9.38,1.87);(9.38,1.87)"
%	 />
%<ellipse fill-style= "solid"
%	 stroke-width= "0.45"
%	 p3= "(2.81,-4.06)"
%	 p2= "(2.81,-7.19)"
%	 p1= "(5.94,-7.19)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.45"
%	 points= "(-0.63,7.5);(-0.63,7.5);(-0.62,1.25);(-0.62,1.25);(-0.62,1.25);(-0.62,-0.63);
%	(-0.62,-0.63);(-0.62,-0.63);(3.13,-4.38);(3.13,-4.38)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.45"
%	 points= "(9.38,-0.62);(9.38,-0.62);(4.38,-5.62);(4.38,-5.62);(4.38,-5.62);(4.38,-5.62);
%	(4.38,-5.62);(4.38,-5.62);(4.38,-5.62);(4.38,-5.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.45"
%	 points= "(4.38,-6.88);(4.38,-6.88);(4.38,-10);(4.38,-10);(4.38,-10);(4.38,-10.62);
%	(4.38,-10.62);(4.38,-10.62);(4.38,-10);(4.38,-10)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(15.63,8.12)(0,0)
\linethickness{0.45mm}
\put(10.62,0.62){\circle*{3.13}}

\linethickness{0.45mm}
\put(15.62,7.5){\line(0,1){0.62}}
\multiput(15.62,7.5)(0.01,-1.88){1}{\line(0,-1){1.88}}
\multiput(11.88,1.87)(0.12,0.12){31}{\line(1,0){0.12}}
\linethickness{0.45mm}
\put(5.62,7.5){\line(0,1){0.62}}
\multiput(5.62,7.5)(0.01,-1.88){1}{\line(0,-1){1.88}}
\multiput(5.63,5.62)(0.12,-0.12){31}{\line(1,0){0.12}}
\linethickness{0.45mm}
\put(4.38,-5.62){\circle*{3.13}}

\linethickness{0.45mm}
\multiput(-0.63,7.5)(0.01,-6.25){1}{\line(0,-1){6.25}}
\put(-0.62,-0.63){\line(0,1){1.88}}
\multiput(-0.62,-0.63)(0.12,-0.12){31}{\line(1,0){0.12}}
\linethickness{0.45mm}
\multiput(4.38,-5.62)(0.12,0.12){42}{\line(1,0){0.12}}
\qbezier(4.38,-5.62)(4.38,-5.62)(4.38,-5.62)
\qbezier(4.38,-5.62)(4.38,-5.62)(4.38,-5.62)
\qbezier(4.38,-5.62)(4.38,-5.62)(4.38,-5.62)
\qbezier(4.38,-5.62)(4.38,-5.62)(4.38,-5.62)
\linethickness{0.45mm}
\put(4.38,-10){\line(0,1){3.12}}
\put(4.38,-10.62){\line(0,1){0.62}}
\put(4.38,-10.62){\line(0,1){0.62}}
\end{picture}


==> PICS/cmn-right.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Sep 02 17:32:58 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.63" x-max="15.63" y-min="-10.62" y-max="8.12" auto-bounding="true">
%<ellipse p3= "(9.06,2.19)"
%	 p2= "(9.06,-0.94)"
%	 p1= "(12.19,-0.94)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(15.62,8.12);(15.62,8.12);(15.62,7.5);(15.62,7.5);(15.62,7.5);(15.63,5.62);
%	(15.63,5.62);(15.63,5.62);(11.88,1.87);(11.88,1.87)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(5.62,8.12);(5.62,8.12);(5.62,7.5);(5.62,7.5);(5.62,7.5);(5.63,5.62);
%	(5.63,5.62);(5.63,5.62);(9.38,1.87);(9.38,1.87)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(2.81,-4.06)"
%	 p2= "(2.81,-7.19)"
%	 p1= "(5.94,-7.19)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(-0.63,7.5);(-0.63,7.5);(-0.62,1.25);(-0.62,1.25);(-0.62,1.25);(-0.62,-0.63);
%	(-0.62,-0.63);(-0.62,-0.63);(3.13,-4.38);(3.13,-4.38)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(9.38,-0.62);(9.38,-0.62);(4.38,-5.62);(4.38,-5.62);(4.38,-5.62);(4.38,-5.62);
%	(4.38,-5.62);(4.38,-5.62);(4.38,-5.62);(4.38,-5.62)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(4.38,-6.88);(4.38,-6.88);(4.38,-10);(4.38,-10);(4.38,-10);(4.38,-10.62);
%	(4.38,-10.62);(4.38,-10.62);(4.38,-10);(4.38,-10)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(15.63,8.12)
\rput{0}(10.62,0.62){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(15.62,8.12)
(15.62,7.5)
(15.63,5.62)(11.88,1.87)
\psline(5.62,8.12)
(5.62,7.5)
(5.63,5.62)(9.38,1.87)
\rput{0}(4.38,-5.62){\psellipse[fillstyle=solid](0,0)(1.57,-1.57)}
\psline(-0.63,7.5)
(-0.62,1.25)
(-0.62,-0.63)(3.13,-4.38)
\pscustom[]{\psline(9.38,-0.62)(4.38,-5.62)
\psbezier(4.38,-5.62)(4.38,-5.62)(4.38,-5.62)
\psbezier(4.38,-5.62)(4.38,-5.62)(4.38,-5.62)
}
\psline(4.38,-6.88)
(4.38,-10)
(4.38,-10.62)(4.38,-10)
\end{pspicture}


==> PICS/comp-caus-0.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Apr 28 20:55:41 GMT+00:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="190" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,70);(0,70);(50,70);(50,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,70);(0,70);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(50,40);(50,40);(50,70);(50,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,95);(15,95);(15,70);(15,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,40);(0,40);(50,40);(50,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,40);(10,40);(10,15);(10,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,70);(110,70);(190,70);(190,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,50);(110,50);(110,20);(110,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(190,40);(190,40);(190,70);(190,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(175,95);(175,95);(175,70);(175,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(165,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(165,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(140,40);(140,40);(190,40);(190,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(165,40);(165,40);(165,15);(165,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,20);(110,20);(140,20);(140,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(158.12,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(120,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,50);(110,50);(140,20);(140,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(125,55);(125,55);(125,35);(125,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,70);(110,70);(140,40);(140,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,95);(35,95);(35,70);(35,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,40);(40,40);(40,15);(40,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,40);(25,40);(25,15);(25,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(180,40);(180,40);(180,15);(180,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(150,40);(150,40);(150,15);(150,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(155,95);(155,95);(155,70);(155,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(126.25,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\dee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(162.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceethree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(157.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceethree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eetwo$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(190,110)
\psline[linewidth=0.75](0,70)(50,70)
\psline[linewidth=0.75](0,70)(0,40)
\psline[linewidth=0.75](50,40)(50,70)
\psline[linewidth=0.75](15,95)(15,70)
\rput(25,110){$\nameslang$}
\rput(25,0){$\inputt$}
\psline[linewidth=0.75](0,40)(50,40)
\psline[linewidth=0.75](10,40)(10,15)
\rput(25,55){\machine}
\psline[linewidth=0.75](110,70)(190,70)
\psline[linewidth=0.75](110,50)(110,20)
\psline[linewidth=0.75](190,40)(190,70)
\psline[linewidth=0.75](175,95)(175,70)
\rput(165,110){$\nameslang$}
\rput(165,0){$\inputt$}
\psline[linewidth=0.75](140,40)(190,40)
\psline[linewidth=0.75](165,40)(165,15)
\psline[linewidth=0.75](110,20)(140,20)
\rput(158.12,55){\universal}
\rput(120,27.5){\program}
\psline[linewidth=0.75](110,50)(140,20)
\psline[linewidth=0.75](125,55)(125,35)
\psline[linewidth=0.75](110,70)(140,40)
\psline[linewidth=0.75](35,95)(35,70)
\psline[linewidth=0.75](40,40)(40,15)
\psline[linewidth=0.75](25,40)(25,15)
\psline[linewidth=0.75](180,40)(180,15)
\psline[linewidth=0.75](150,40)(150,15)
\psline[linewidth=0.75](155,95)(155,70)
\rput[l](126.25,40){$\dee$}
\rput[r](147.5,15){$\ceeone$}
\rput[r](162.5,15){$\ceetwo$}
\rput[r](177.5,15){$\ceethree$}
\rput[l](157.5,95){$\eeone$}
\rput[l](177.5,95){$\eetwo$}
\rput[r](7.5,15){$\ceeone$}
\rput[r](22.5,15){$\ceetwo$}
\rput[r](37.5,15){$\ceethree$}
\rput[l](17.5,95){$\eeone$}
\rput[l](37.5,95){$\eetwo$}
\end{pspicture}


==> PICS/comp-caus-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Apr 29 06:50:25 GMT+00:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="190" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,70);(110,70);(190,70);(190,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(190,40);(190,40);(190,70);(190,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(175,95);(175,95);(175,70);(175,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(165,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(165,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(140,40);(140,40);(190,40);(190,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(165,40);(165,40);(165,15);(165,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(158.12,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(125,55);(125,55);(125,15);(125,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,70);(110,70);(140,40);(140,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(180,40);(180,40);(180,15);(180,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(150,40);(150,40);(150,15);(150,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(155,95);(155,95);(155,70);(155,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\description$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(123.75,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\dee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(162.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceethree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(157.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(0,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(0,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(190,110)
\psline[linewidth=0.75](110,70)(190,70)
\psline[linewidth=0.75](190,40)(190,70)
\psline[linewidth=0.75](175,95)(175,70)
\rput(165,110){$\nameslang$}
\rput(165,0){$\inputt$}
\psline[linewidth=0.75](140,40)(190,40)
\psline[linewidth=0.75](165,40)(165,15)
\rput(158.12,55){\universal}
\psline[linewidth=0.75](125,55)(125,15)
\psline[linewidth=0.75](110,70)(140,40)
\psline[linewidth=0.75](180,40)(180,15)
\psline[linewidth=0.75](150,40)(150,15)
\psline[linewidth=0.75](155,95)(155,70)
\rput(125,0){$\description$}
\rput[r](123.75,15){$\dee$}
\rput[r](147.5,15){$\ceeone$}
\rput[r](162.5,15){$\ceetwo$}
\rput[r](177.5,15){$\ceethree$}
\rput[l](157.5,95){$\eeone$}
\rput[l](177.5,95){$\eetwo$}
\rput(0,110){\nothing}
\rput(0,0){\nothing}
\end{pspicture}


==> PICS/comp-caus-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Apr 28 21:03:37 GMT+00:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="190" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,70);(0,70);(50,70);(50,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,70);(0,70);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(50,40);(50,40);(50,70);(50,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,95);(15,95);(15,70);(15,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,40);(0,40);(50,40);(50,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,40);(10,40);(10,15);(10,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,95);(35,95);(35,70);(35,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,40);(40,40);(40,15);(40,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,40);(25,40);(25,15);(25,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceethree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,93.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,93.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eetwo$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(190,110)
\psline[linewidth=0.75](0,70)(50,70)
\psline[linewidth=0.75](0,70)(0,40)
\psline[linewidth=0.75](50,40)(50,70)
\psline[linewidth=0.75](15,95)(15,70)
\rput(25,110){$\nameslang$}
\rput(25,0){$\inputt$}
\psline[linewidth=0.75](0,40)(50,40)
\psline[linewidth=0.75](10,40)(10,15)
\rput(25,55){\machine}
\psline[linewidth=0.75](35,95)(35,70)
\psline[linewidth=0.75](40,40)(40,15)
\psline[linewidth=0.75](25,40)(25,15)
\rput(190,110){\nothing}
\rput(190,0){\nothing}
\rput[r](7.5,13.75){$\ceeone$}
\rput[r](22.5,13.75){$\ceetwo$}
\rput[r](37.5,13.75){$\ceethree$}
\rput[l](17.5,93.75){$\eeone$}
\rput[l](37.5,93.75){$\eetwo$}
\end{pspicture}


==> PICS/comp-caus.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Apr 28 20:57:11 GMT+00:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="190" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,70);(0,70);(50,70);(50,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,70);(0,70);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(50,40);(50,40);(50,70);(50,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,95);(15,95);(15,70);(15,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,40);(0,40);(50,40);(50,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,40);(10,40);(10,15);(10,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,70);(110,70);(190,70);(190,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,50);(110,50);(110,20);(110,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(190,40);(190,40);(190,70);(190,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(175,95);(175,95);(175,70);(175,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(165,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(165,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(140,40);(140,40);(190,40);(190,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(165,40);(165,40);(165,15);(165,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,20);(110,20);(140,20);(140,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(158.12,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(120,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(85,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,50);(110,50);(140,20);(140,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(125,55);(125,55);(125,35);(125,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,70);(110,70);(140,40);(140,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,95);(35,95);(35,70);(35,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,40);(40,40);(40,15);(40,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,40);(25,40);(25,15);(25,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(180,40);(180,40);(180,15);(180,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(150,40);(150,40);(150,15);(150,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(155,95);(155,95);(155,70);(155,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(126.25,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\dee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(162.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceethree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(157.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceethree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eetwo$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(190,110)
\psline[linewidth=0.75](0,70)(50,70)
\psline[linewidth=0.75](0,70)(0,40)
\psline[linewidth=0.75](50,40)(50,70)
\psline[linewidth=0.75](15,95)(15,70)
\rput(25,110){$\nameslang$}
\rput(25,0){$\inputt$}
\psline[linewidth=0.75](0,40)(50,40)
\psline[linewidth=0.75](10,40)(10,15)
\rput(25,55){\machine}
\psline[linewidth=0.75](110,70)(190,70)
\psline[linewidth=0.75](110,50)(110,20)
\psline[linewidth=0.75](190,40)(190,70)
\psline[linewidth=0.75](175,95)(175,70)
\rput(165,110){$\nameslang$}
\rput(165,0){$\inputt$}
\psline[linewidth=0.75](140,40)(190,40)
\psline[linewidth=0.75](165,40)(165,15)
\psline[linewidth=0.75](110,20)(140,20)
\rput(158.12,55){\universal}
\rput(120,27.5){\program}
\rput(85,55){\EQLS}
\psline[linewidth=0.75](110,50)(140,20)
\psline[linewidth=0.75](125,55)(125,35)
\psline[linewidth=0.75](110,70)(140,40)
\psline[linewidth=0.75](35,95)(35,70)
\psline[linewidth=0.75](40,40)(40,15)
\psline[linewidth=0.75](25,40)(25,15)
\psline[linewidth=0.75](180,40)(180,15)
\psline[linewidth=0.75](150,40)(150,15)
\psline[linewidth=0.75](155,95)(155,70)
\rput[l](126.25,40){$\dee$}
\rput[r](147.5,15){$\ceeone$}
\rput[r](162.5,15){$\ceetwo$}
\rput[r](177.5,15){$\ceethree$}
\rput[l](157.5,95){$\eeone$}
\rput[l](177.5,95){$\eetwo$}
\rput[r](7.5,15){$\ceeone$}
\rput[r](22.5,15){$\ceetwo$}
\rput[r](37.5,15){$\ceethree$}
\rput[l](17.5,95){$\eeone$}
\rput[l](37.5,95){$\eetwo$}
\end{pspicture}


==> PICS/comp-part.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Apr 28 21:00:08 GMT+00:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-7.5" x-max="202.5" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(132.5,70);(132.5,70);(202.5,70);(202.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(202.5,40);(202.5,40);(202.5,70);(202.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(192.5,95);(192.5,95);(192.5,70);(192.5,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(181.25,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(172.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(162.5,40);(162.5,40);(202.5,40);(202.5,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(172.5,40);(172.5,40);(172.5,15);(172.5,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(176.25,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(100,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(127.5,40);(127.5,40);(127.5,15);(127.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(112.5,55);(112.5,55);(142.5,25);(142.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(192.5,40);(192.5,40);(192.5,15);(192.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(152.5,25);(152.5,25);(152.5,15);(152.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(172.5,95);(172.5,95);(172.5,70);(172.5,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(127.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\descriptionn$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(-7.5,70);(-7.5,70);(82.5,70);(82.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(82.5,40);(82.5,40);(82.5,70);(82.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(62.5,95);(62.5,95);(62.5,70);(62.5,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(52.5,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(52.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(22.5,40);(22.5,40);(82.5,40);(82.5,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(52.5,40);(52.5,40);(52.5,15);(52.5,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(46.25,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(7.5,55);(7.5,55);(7.5,15);(7.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(-7.5,70);(-7.5,70);(22.5,40);(22.5,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(72.5,40);(72.5,40);(72.5,15);(72.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(32.5,40);(32.5,40);(32.5,15);(32.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(42.5,95);(42.5,95);(42.5,70);(42.5,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\descriptionn$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(142.5,25);(142.5,25);(162.5,25);(162.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(112.5,55);(112.5,55);(132.5,55);(132.5,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(132.5,55);(132.5,55);(162.5,25);(162.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(132.5,70);(132.5,70);(162.5,40);(162.5,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(147.5,55);(147.5,55);(147.5,40);(147.5,40)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(137.5,40)"
%	 text-rotation= "-45"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\partial
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\dee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(31.25,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(51.25,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(71.25,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceethree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(195,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\dee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(151.25,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceeone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(171.25,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceetwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(191.25,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ceethree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(148.75,43.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\dee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(202.5,110)
\psline[linewidth=0.75](132.5,70)(202.5,70)
\psline[linewidth=0.75](202.5,40)(202.5,70)
\psline[linewidth=0.75](192.5,95)(192.5,70)
\rput(181.25,110){$\nameslang$}
\rput(172.5,0){$\inputt$}
\psline[linewidth=0.75](162.5,40)(202.5,40)
\psline[linewidth=0.75](172.5,40)(172.5,15)
\rput(176.25,55){\universal}
\rput(100,55){\EQLS}
\psline[linewidth=0.75](127.5,40)(127.5,15)
\psline[linewidth=0.75](112.5,55)(142.5,25)
\psline[linewidth=0.75](192.5,40)(192.5,15)
\psline[linewidth=0.75](152.5,25)(152.5,15)
\psline[linewidth=0.75](172.5,95)(172.5,70)
\rput(127.5,0){$\descriptionn$}
\psline[linewidth=0.75](-7.5,70)(82.5,70)
\psline[linewidth=0.75](82.5,40)(82.5,70)
\psline[linewidth=0.75](62.5,95)(62.5,70)
\rput(52.5,110){$\nameslang$}
\rput(52.5,0){$\inputt$}
\psline[linewidth=0.75](22.5,40)(82.5,40)
\psline[linewidth=0.75](52.5,40)(52.5,15)
\rput(46.25,55){\universal}
\psline[linewidth=0.75](7.5,55)(7.5,15)
\psline[linewidth=0.75](-7.5,70)(22.5,40)
\psline[linewidth=0.75](72.5,40)(72.5,15)
\psline[linewidth=0.75](32.5,40)(32.5,15)
\psline[linewidth=0.75](42.5,95)(42.5,70)
\rput(7.5,0){$\descriptionn$}
\psline[linewidth=0.75](142.5,25)(162.5,25)
\psline[linewidth=0.75](112.5,55)(132.5,55)
\psline[linewidth=0.75](132.5,55)(162.5,25)
\psline[linewidth=0.75](132.5,70)(162.5,40)
\psline[linewidth=0.75](147.5,55)(147.5,40)
\rput{-45}(137.5,40){\partial}
\rput[r](5,15){$\dee$}
\rput[r](31.25,15){$\ceeone$}
\rput[r](51.25,15){$\ceetwo$}
\rput[r](71.25,15){$\ceethree$}
\rput[l](45,95){$\eeone$}
\rput[l](65,95){$\eetwo$}
\rput[l](175,95){$\eeone$}
\rput[l](195,95){$\eetwo$}
\rput[r](125,16.25){$\dee$}
\rput[r](151.25,16.25){$\ceeone$}
\rput[r](171.25,16.25){$\ceetwo$}
\rput[r](191.25,16.25){$\ceethree$}
\rput[l](148.75,43.75){$\dee$}
\end{pspicture}


==> PICS/comp.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 13 16:23:02 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="1.25" y-max="71.25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(40,47.5);(40,47.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(0,22.5);(0,22.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,22.5);(40,22.5);(40,47.5);(40,47.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,65);(20,65);(20,47.5);(20,47.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,71.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,22.5);(0,22.5);(40,22.5);(40,22.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,22.5);(30,22.5);(30,7.5);(30,7.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,53.12);(70,53.12);(130,53.12);(130,53.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,41.25);(70,41.25);(70,16.25);(70,16.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,28.12);(130,28.12);(130,53.12);(130,53.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,65);(110,65);(110,53.12);(110,53.12)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,71.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,28.12);(95,28.12);(130,28.12);(130,28.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,28.12);(110,28.12);(110,7.5);(110,7.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,16.25);(70,16.25);(95,16.25);(95,16.25)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(108.12,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(75,23.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,41.25);(70,41.25);(95,16.25);(95,16.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(83.12,40);(83.12,40);(83.12,28.12);(83.12,28.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,53.12);(70,53.12);(95,28.12);(95,28.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,22.5);(10,22.5);(10,7.5);(10,7.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,15);(80,15);(80,7.5);(80,7.5)"
%	 stroke-width= "0.75"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(130,71.25)
\psline[linewidth=0.75](0,47.5)(40,47.5)
\psline[linewidth=0.75](0,47.5)(0,22.5)
\psline[linewidth=0.75](40,22.5)(40,47.5)
\psline[linewidth=0.75](20,65)(20,47.5)
\rput(20,71.25){$\nameslang$}
\rput(30,1.25){$\inputt$}
\psline[linewidth=0.75](0,22.5)(40,22.5)
\psline[linewidth=0.75](30,22.5)(30,7.5)
\rput(20,35){\machine}
\psline[linewidth=0.75](70,53.12)(130,53.12)
\psline[linewidth=0.75](70,41.25)(70,16.25)
\psline[linewidth=0.75](130,28.12)(130,53.12)
\psline[linewidth=0.75](110,65)(110,53.12)
\rput(110,71.25){$\nameslang$}
\rput(110,1.25){$\inputt$}
\psline[linewidth=0.75](95,28.12)(130,28.12)
\psline[linewidth=0.75](110,28.12)(110,7.5)
\psline[linewidth=0.75](70,16.25)(95,16.25)
\rput(108.12,40){\universal}
\rput(75,23.75){\program}
\rput(55,35){\EQLS}
\psline[linewidth=0.75](70,41.25)(95,16.25)
\psline[linewidth=0.75](83.12,40)(83.12,28.12)
\psline[linewidth=0.75](70,53.12)(95,28.12)
\psline[linewidth=0.75](10,22.5)(10,7.5)
\psline[linewidth=0.75](80,15)(80,7.5)
\end{pspicture}


==> PICS/computation-tight.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Apr 29 04:13:13 GMT+00:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="305" y-min="30" y-max="90" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(100,60);(100,60);(100,30);(100,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(125,60);(125,60);(125,30);(125,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(95,60);(95,60);(75,80);(75,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(75,80);(75,80);(130,80);(130,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(95,60);(95,60);(130,60);(130,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(130,80);(130,80);(130,60);(130,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,90);(110,90);(110,80);(110,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(85,70);(85,70);(85,57.5);(85,57.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(167.5,57.5);(167.5,57.5);(167.5,45);(167.5,45)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(185,47.5);(185,47.5);(185,30);(185,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(157.5,67.5);(157.5,67.5);(177.5,67.5);(177.5,67.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(197.5,47.5);(197.5,47.5);(177.5,47.5);(177.5,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(197.5,60);(197.5,60);(177.5,80);(177.5,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(177.5,67.5);(177.5,67.5);(197.5,47.5);(197.5,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(177.5,80);(177.5,80);(217.5,80);(217.5,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(187.5,70);(187.5,70);(187.5,57.5);(187.5,57.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(197.5,60);(197.5,60);(217.5,60);(217.5,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(217.5,80);(217.5,80);(217.5,60);(217.5,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(157.5,67.5);(157.5,67.5);(177.5,47.5);(177.5,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(197.5,90);(197.5,90);(197.5,80);(197.5,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(185,67.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(207.5,60);(207.5,60);(207.5,30);(207.5,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,57.5)"
%	 text-rotation= "-45"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partial$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(203.75,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(97.5,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(120,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(112.5,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(200,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(205,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(182.5,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(110,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universalmkn$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(157.5,55);(157.5,55);(157.5,35);(157.5,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(157.5,35);(157.5,35);(177.5,35);(177.5,35)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(165,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(157.5,55);(157.5,55);(177.5,35);(177.5,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(75,47.5);(75,47.5);(95,47.5);(95,47.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(82.5,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(75,67.5);(75,67.5);(95,47.5);(95,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(75,67.5);(75,67.5);(75,47.5);(75,47.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(165,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(82.5,67.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,60);(40,60);(40,30);(40,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,60);(0,60);(0,80);(0,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,80);(0,80);(50,80);(50,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,60);(0,60);(50,60);(50,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(50,80);(50,80);(50,60);(50,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,88.75);(25,88.75);(25,80);(25,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(7.5,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(37.5,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(27.5,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(25,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,60);(10,60);(10,30);(10,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(292.5,60);(292.5,60);(292.5,30);(292.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(245,47.5);(245,47.5);(245,67.5);(245,67.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(265,80);(265,80);(305,80);(305,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(285,60);(285,60);(305,60);(305,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(305,80);(305,80);(305,60);(305,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(287.5,90);(287.5,90);(287.5,80);(287.5,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(257.5,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(290,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.8"
%	 anchor-point= "(290,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(260,47.5);(260,47.5);(260,30);(260,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(285,60);(285,60);(265,80);(265,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(245,47.5);(245,47.5);(285,47.5);(285,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(245,67.5);(245,67.5);(265,67.5);(265,67.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(285,47.5);(285,47.5);(265,67.5);(265,67.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(275,70);(275,70);(275,57.5);(275,57.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(272.5,67.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(233.75,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsc$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(63.75,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsa$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(291.25,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(258.75,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Gx$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(305,90)
\psline[linewidth=0.75](100,60)(100,30)
\psline[linewidth=0.75](125,60)(125,30)
\psline[linewidth=0.75](95,60)(75,80)
\psline[linewidth=0.75](75,80)(130,80)
\psline[linewidth=0.75](95,60)(130,60)
\psline[linewidth=0.75](130,80)(130,60)
\psline[linewidth=0.75](110,90)(110,80)
\psline[linewidth=0.75](85,70)(85,57.5)
\psline[linewidth=0.75](167.5,57.5)(167.5,45)
\psline[linewidth=0.75](185,47.5)(185,30)
\psline[linewidth=0.75](157.5,67.5)(177.5,67.5)
\psline[linewidth=0.75](197.5,47.5)(177.5,47.5)
\psline[linewidth=0.75](197.5,60)(177.5,80)
\psline[linewidth=0.75](177.5,67.5)(197.5,47.5)
\psline[linewidth=0.75](177.5,80)(217.5,80)
\psline[linewidth=0.75](187.5,70)(187.5,57.5)
\psline[linewidth=0.75](197.5,60)(217.5,60)
\psline[linewidth=0.75](217.5,80)(217.5,60)
\psline[linewidth=0.75](157.5,67.5)(177.5,47.5)
\psline[linewidth=0.75](197.5,90)(197.5,80)
\rput[r](185,67.5){$\Progtype$}
\psline[linewidth=0.75](207.5,60)(207.5,30)
\rput{-45}(177.5,57.5){$\partial$}
\rput(203.75,70){$\universal$}
\rput[r](97.5,31.25){$\Progk$}
\rput[r](120,31.25){$\Progm$}
\rput[l](112.5,88.75){$\Progn$}
\rput[l](200,88.75){$\Progn$}
\rput[r](205,31.25){$\Progm$}
\rput[r](182.5,31.25){$\Progk$}
\rput(110,70){$\universalmkn$}
\psline[linewidth=0.75](157.5,55)(157.5,35)
\psline[linewidth=0.75](157.5,35)(177.5,35)
\rput(165,40){\program}
\psline[linewidth=0.75](157.5,55)(177.5,35)
\psline[linewidth=0.75](75,47.5)(95,47.5)
\rput(82.5,52.5){\program}
\psline[linewidth=0.75](75,67.5)(95,47.5)
\psline[linewidth=0.75](75,67.5)(75,47.5)
\rput[r](165,55){$\Progtype$}
\rput[r](82.5,67.5){$\Progtype$}
\psline[linewidth=0.75](40,60)(40,30)
\psline[linewidth=0.75](0,60)(0,80)
\psline[linewidth=0.75](0,80)(50,80)
\psline[linewidth=0.75](0,60)(50,60)
\psline[linewidth=0.75](50,80)(50,60)
\psline[linewidth=0.75](25,88.75)(25,80)
\rput[r](7.5,31.25){$\Progk$}
\rput[r](37.5,31.25){$\Progm$}
\rput[l](27.5,88.75){$\Progn$}
\rput(25,70){\gee}
\psline[linewidth=0.75](10,60)(10,30)
\psline[linewidth=0.75](292.5,60)(292.5,30)
\psline[linewidth=0.75](245,47.5)(245,67.5)
\psline[linewidth=0.75](265,80)(305,80)
\psline[linewidth=0.75](285,60)(305,60)
\psline[linewidth=0.75](305,80)(305,60)
\psline[linewidth=0.75](287.5,90)(287.5,80)
\rput[r](257.5,31.25){$\Progk$}
\rput[r](290,31.25){$\Progm$}
\rput[l](290,88.75){$\Progn$}
\psline[linewidth=0.75](260,47.5)(260,30)
\psline[linewidth=0.75](285,60)(265,80)
\psline[linewidth=0.75](245,47.5)(285,47.5)
\psline[linewidth=0.75](245,67.5)(265,67.5)
\psline[linewidth=0.75](285,47.5)(265,67.5)
\psline[linewidth=0.75](275,70)(275,57.5)
\rput[r](272.5,67.5){$\Progtype$}
\rput(145,70){$\eqlsb$}
\rput(233.75,70){$\eqlsc$}
\rput(63.75,70){$\eqlsa$}
\rput(291.25,70){$\universal$}
\rput(258.75,57.5){$\Gx$}
\end{pspicture}


==> PICS/cun-left.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Sep 02 17:29:59 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-2.19" x-max="10" y-min="-10.62" y-max="8.12" auto-bounding="true">
%<multicurve points= "(0.62,0);(0.62,0);(5.62,-5);(5.62,-5);(5.62,-5);(4.38,-5);
%	(4.38,-5);(4.38,-5);(5,-5);(5,-5)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(-2.19,2.81)"
%	 p2= "(-2.19,-0.31)"
%	 p1= "(0.94,-0.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(3.75,-3.13)"
%	 p2= "(3.75,-6.25)"
%	 p1= "(6.88,-6.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(10,8.12);(10,8.12);(10,5.62);(10,5.62);(10,5.62);(10,0);
%	(10,0);(10,0);(6.25,-3.75);(6.25,-3.75)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(5,-6.25);(5,-6.25);(5,-10);(5,-10);(5,-10);(5,-10.62);
%	(5,-10.62);(5,-10.62);(5,-10);(5,-10)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(10,8.12)
\psline(0.62,0)
(5.62,-5)
(4.38,-5)(5,-5)
\rput{0}(-0.62,1.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(5.31,-4.69){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(10,8.12)
(10,5.62)
(10,0)(6.25,-3.75)
\psline(5,-6.25)
(5,-10)
(5,-10.62)(5,-10)
\end{pspicture}


==> PICS/cun-right.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Sep 02 17:34:38 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.63" x-max="12.19" y-min="-10.62" y-max="8.12" auto-bounding="true">
%<ellipse p3= "(9.06,2.81)"
%	 p2= "(9.06,-0.31)"
%	 p1= "(12.19,-0.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(2.81,-3.44)"
%	 p2= "(2.81,-6.56)"
%	 p1= "(5.94,-6.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(4.38,-6.25);(4.38,-6.25);(4.38,-10);(4.38,-10);(4.38,-10);(4.38,-10.62);
%	(4.38,-10.62);(4.38,-10.62);(4.38,-10);(4.38,-10)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(-0.63,8.12);(-0.63,8.12);(-0.62,1.87);(-0.62,1.87);(-0.62,1.87);(-0.62,0);
%	(-0.62,0);(-0.62,0);(3.13,-3.75);(3.13,-3.75)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(9.38,0);(9.38,0);(4.38,-5);(4.38,-5);(4.38,-5);(4.38,-5);
%	(4.38,-5);(4.38,-5);(4.38,-5);(4.38,-5)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(12.19,8.12)
\rput{0}(10.62,1.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(4.38,-5){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(4.38,-6.25)
(4.38,-10)
(4.38,-10.62)(4.38,-10)
\psline(-0.63,8.12)
(-0.62,1.87)
(-0.62,0)(3.13,-3.75)
\pscustom[]{\psline(9.38,0)(4.38,-5)
\psbezier(4.38,-5)(4.38,-5)(4.38,-5)
\psbezier(4.38,-5)(4.38,-5)(4.38,-5)
}
\end{pspicture}


==> PICS/curved.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jan 08 11:25:32 GMT 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="140" y-min="0" y-max="45" auto-bounding="true">
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 points= "(10,20);(10,20);(15,30);(20,25);(25,20);(25,0);
%	(35,10);(45,20);(55,20);(65,15);(75,10);(65,25);
%	(80,30);(95,35);(80,45);(100,45);(120,45);(105,45);
%	(120,40);(135,35);(125,45);(130,30);(135,15);(140,20);
%	(140,20);(140,20);(140,20);(140,20);(140,20);(140,20);
%	(140,20)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(140,45)
\pscustom[linewidth=0.4]{\psbezier(10,20)(10,20)(15,30)(20,25)
\psbezier(25,20)(25,0)(35,10)
\psbezier(45,20)(55,20)(65,15)
\psbezier(75,10)(65,25)(80,30)
\psbezier(95,35)(80,45)(100,45)
\psbezier(120,45)(105,45)(120,40)
\psbezier(135,35)(125,45)(130,30)
\psbezier(135,15)(140,20)(140,20)
\psbezier(140,20)(140,20)(140,20)
\psbezier(140,20)(140,20)(140,20)
}
\end{pspicture}


==> PICS/dataserv.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Mar 16 16:45:41 GMT-10:00 2023
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="77.5" y-min="0" y-max="44.07" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "1.25"
%	 points= "(70,40);(70,40);(70,0);(70,0)"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 stroke-width= "1.25"
%	 p3= "(74.07,35.93)"
%	 p2= "(74.07,44.07)"
%	 p1= "(65.93,44.07)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "1.25"
%	 points= "(30,30);(30,30);(15,15);(15,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "1.25"
%	 points= "(15,15);(15,15);(15,0);(15,0)"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 stroke-width= "1.25"
%	 p3= "(18.79,11.21)"
%	 p2= "(18.79,18.79)"
%	 p1= "(11.21,18.79)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "1.25"
%	 points= "(0,30);(0,30);(15,15);(15,15)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "1.25"
%	 text-vert-align= "center-v"
%	 anchor-point= "(12.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 stroke-width= "1.25"
%	 text-vert-align= "center-v"
%	 anchor-point= "(67.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "1.25"
%	 points= "(0,40);(0,40);(0,30);(0,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "1.25"
%	 points= "(30,40);(30,40);(30,30);(30,30)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "1.25"
%	 text-vert-align= "center-v"
%	 anchor-point= "(32.5,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 stroke-width= "1.25"
%	 text-vert-align= "center-v"
%	 anchor-point= "(2.5,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 stroke-width= "1.25"
%	 text-vert-align= "center-v"
%	 anchor-point= "(77.5,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\delete$
%</text>
%<text fill-style= "none"
%	 stroke-width= "1.25"
%	 text-vert-align= "center-v"
%	 anchor-point= "(21.25,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ccopy$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(77.5,44.07)
\psline[linewidth=1.25](70,40)(70,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(70,40){\psellipse[linewidth=1.25,fillcolor=userFillColour,fillstyle=solid](0,0)(4.07,-4.07)}
\psline[linewidth=1.25](30,30)(15,15)
\psline[linewidth=1.25](15,15)(15,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(15,15){\psellipse[linewidth=1.25,fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=1.25](0,30)(15,15)
\rput[r](12.5,0){$\AAh$}
\rput[r](67.5,0){$\AAh$}
\psline[linewidth=1.25](0,40)(0,30)
\psline[linewidth=1.25](30,40)(30,30)
\rput[l](32.5,40){$\AAh$}
\rput[l](2.5,40){$\AAh$}
\rput[l](77.5,40){$\delete$}
\rput[l](21.25,15){$\ccopy$}
\end{pspicture}


==> PICS/eval.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon May 17 23:15:37 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="200" y-min="0" y-max="150" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(80,80);(80,80);(80,40);(80,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,40);(80,40);(0,40);(0,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(80,80);(80,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,40);(60,40);(60,0);(60,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,120);(40,120);(40,80);(40,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(0,40);(0,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(20,0);(20,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,100);(200,100);(200,60);(200,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,20);(160,20);(120,20);(120,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,100);(120,100);(200,100);(200,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,60);(180,60);(180,0);(180,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,120);(160,120);(160,100);(160,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,60);(120,60);(120,20);(120,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,20);(140,20);(140,0);(140,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,60);(200,60);(160,60);(160,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,100);(120,100);(160,60);(160,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,60);(120,60);(160,20);(160,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,40);(140,40);(140,80);(140,80)"
%	 stroke-width= "1.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(170,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(136.25,65)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Code$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165,117.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,117.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,31.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,150)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\LHS$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RHS$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(200,150)
\psline[linewidth=0.75](80,80)(80,40)
\psline[linewidth=0.75](80,40)(0,40)
\psline[linewidth=0.75](0,80)(80,80)
\psline[linewidth=0.75](60,40)(60,0)
\psline[linewidth=0.75](40,120)(40,80)
\psline[linewidth=0.75](0,80)(0,40)
\psline[linewidth=0.75](20,40)(20,0)
\psline[linewidth=0.75](200,100)(200,60)
\psline[linewidth=0.75](160,20)(120,20)
\psline[linewidth=0.75](120,100)(200,100)
\psline[linewidth=0.75](180,60)(180,0)
\psline[linewidth=0.75](160,120)(160,100)
\psline[linewidth=0.75](120,60)(120,20)
\psline[linewidth=0.75](140,20)(140,0)
\psline[linewidth=0.75](200,60)(160,60)
\psline[linewidth=0.75](120,100)(160,60)
\psline[linewidth=0.75](120,60)(160,20)
\psline[linewidth=1.4](140,40)(140,80)
\rput(170,80){$\Univ$}
\rput(100,60){\EQLS}
\rput[r](136.25,65){$\Code$}
\rput[l](165,117.5){$\Cee$}
\rput[l](45,117.5){$\Cee$}
\rput[r](15,2.5){$\Aee$}
\rput[r](55,2.5){$\Bee$}
\rput(40,60){$\fee$}
\rput(130,31.25){$\Fee$}
\rput[r](135,2.5){$\Aee$}
\rput[r](175,2.5){$\Bee$}
\rput(100,150){\EQLS}
\rput(40,150){$\LHS$}
\rput(160,150){$\RHS$}
\rput(140,40){$\Dott$}
\end{pspicture}


==> PICS/evalnon.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Mar 16 16:39:13 GMT-10:00 2023
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="220" y-min="0" y-max="120" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(80,80);(80,80);(80,40);(80,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(80,40);(80,40);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(0,80);(0,80);(80,80);(80,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(60,40);(60,40);(60,0);(60,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(40,120);(40,120);(40,80);(40,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(0,80);(0,80);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(20,40);(20,40);(20,0);(20,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(220,100);(220,100);(220,60);(220,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(180,20);(180,20);(140,20);(140,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(140,100);(140,100);(220,100);(220,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(200,60);(200,60);(200,0);(200,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(180,120);(180,120);(180,100);(180,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(140,60);(140,60);(140,20);(140,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(160,20);(160,20);(160,0);(160,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(220,60);(220,60);(180,60);(180,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(140,100);(140,100);(180,60);(180,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(140,60);(140,60);(180,20);(180,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(160,40);(160,40);(160,80);(160,80)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.6"
%	 text-vert-align= "center-v"
%	 anchor-point= "(190,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.6"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.6"
%	 text-vert-align= "center-v"
%	 anchor-point= "(156.25,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Code$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.6"
%	 text-vert-align= "center-v"
%	 anchor-point= "(185,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.6"
%	 text-vert-align= "center-v"
%	 anchor-point= "(45,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.6"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.6"
%	 text-vert-align= "center-v"
%	 anchor-point= "(55,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.6"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.6"
%	 text-vert-align= "center-v"
%	 anchor-point= "(150,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.6"
%	 text-vert-align= "center-v"
%	 anchor-point= "(155,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.6"
%	 text-vert-align= "center-v"
%	 anchor-point= "(195,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.6"
%	 text-vert-align= "center-v"
%	 anchor-point= "(160,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(220,120)
\psline[linewidth=0.6](80,80)(80,40)
\psline[linewidth=0.6](80,40)(0,40)
\psline[linewidth=0.6](0,80)(80,80)
\psline[linewidth=0.6](60,40)(60,0)
\psline[linewidth=0.6](40,120)(40,80)
\psline[linewidth=0.6](0,80)(0,40)
\psline[linewidth=0.6](20,40)(20,0)
\psline[linewidth=0.6](220,100)(220,60)
\psline[linewidth=0.6](180,20)(140,20)
\psline[linewidth=0.6](140,100)(220,100)
\psline[linewidth=0.6](200,60)(200,0)
\psline[linewidth=0.6](180,120)(180,100)
\psline[linewidth=0.6](140,60)(140,20)
\psline[linewidth=0.6](160,20)(160,0)
\psline[linewidth=0.6](220,60)(180,60)
\psline[linewidth=0.6](140,100)(180,60)
\psline[linewidth=0.6](140,60)(180,20)
\psline[linewidth=0.6](160,40)(160,80)
\rput(190,80){$\Univ$}
\rput(110,60){\EQLS}
\rput[r](156.25,65){$\Code$}
\rput[l](185,117.5){$\Cee$}
\rput[l](45,117.5){$\Cee$}
\rput[r](15,2.5){$\Aee$}
\rput[r](55,2.5){$\Bee$}
\rput(40,60){$\fee$}
\rput(150,31.25){$\Fee$}
\rput[r](155,2.5){$\Aee$}
\rput[r](195,2.5){$\Bee$}
\rput(160,40){$\Dott$}
\end{pspicture}


==> PICS/kleene-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Aug 15 13:14:44 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3.75" x-max="173.75" y-min="0" y-max="97.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(113.75,85.62);(113.75,85.62);(173.75,85.62);(173.75,85.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(113.75,51.25);(113.75,51.25);(113.75,26.25);(113.75,26.25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(173.75,60.62);(173.75,60.62);(173.75,85.62);(173.75,85.62)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(153.75,97.5);(153.75,97.5);(153.75,85.62);(153.75,85.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(138.75,60.62);(138.75,60.62);(173.75,60.62);(173.75,60.62)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(165,60.62);(165,60.62);(165,0);(165,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(113.75,26.25);(113.75,26.25);(138.75,26.25);(138.75,26.25)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(151.87,72.5)"
%	 stroke-width= "0.75"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(121.25,33.12)"
%	 stroke-width= "0.75"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(95,71.25)"
%	 stroke-width= "0.75"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(113.75,51.25);(113.75,51.25);(138.75,26.25);(138.75,26.25)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(126.25,73.13);(126.25,73.13);(126.25,39.37);(126.25,39.37)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(113.75,85.62);(113.75,85.62);(138.75,60.62);(138.75,60.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(23.75,85.63);(23.75,85.63);(73.75,85.62);(73.75,85.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(73.75,60.62);(73.75,60.62);(73.75,85.62);(73.75,85.62)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(48.75,97.5);(48.75,97.5);(48.75,85.62);(48.75,85.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(23.75,60.63);(23.75,60.63);(73.75,60.62);(73.75,60.62)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(63.75,60.62);(63.75,60.62);(63.75,0);(63.75,0)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(33.75,60.63);(33.75,60.63);(33.75,39.37);(33.75,39.37)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(23.75,85.63);(23.75,85.63);(23.75,60.63);(23.75,60.63)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(48.75,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(3.75,47.49);(3.75,47.49);(25,47.49);(25,47.49)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(45,27.5);(45,27.5);(23.75,27.5);(23.75,27.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,47.49);(25,47.49);(45,27.5);(45,27.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(3.75,47.49);(3.75,47.49);(23.75,27.5);(23.75,27.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(24.38,10.63);(24.38,10.63);(24.38,0);(24.38,0)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(25.78,9.22)"
%	 p2= "(25.78,12.03)"
%	 p1= "(22.96,12.03)"
%	 fill-color= "#330033"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,27.5);(35,27.5);(35,21.25);(35,21.25)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(14.38,36.88);(14.38,36.88);(14.38,20.01);(14.38,20.01)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,21.25);(35,21.25);(24.38,10.63);(24.38,10.63)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(14.38,20.01);(14.38,20.01);(24.38,10);(24.38,10)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(145,60.62);(145,60.62);(145,0);(145,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,36.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(143.12,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\Beliefs
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(166.88,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Causes
%</text>
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 fill-color= "#ffffff"
%	 anchor-point= "(126.25,55.62)"
%	 text-frame= "rectangle"
%	 text-hor-align= "center-h"
%	 >
%\Beliefs
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(23.12,4.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\Beliefs
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65.62,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Causes
%</text>
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 fill-color= "#ffffff"
%	 anchor-point= "(35,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Beliefs
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(173.75,97.5)
\psline[linewidth=0.75](113.75,85.62)(173.75,85.62)
\psline[linewidth=0.75](113.75,51.25)(113.75,26.25)
\psline[linewidth=0.75](173.75,60.62)(173.75,85.62)
\psline[linewidth=0.75]{<-}(153.75,97.5)(153.75,85.62)
\psline[linewidth=0.75](138.75,60.62)(173.75,60.62)
\psline[linewidth=0.75]{<-}(165,60.62)(165,0)
\psline[linewidth=0.75](113.75,26.25)(138.75,26.25)
\rput(151.87,72.5){\universal}
\rput(121.25,33.12){\program}
\rput(95,71.25){\EQLS}
\psline[linewidth=0.75](113.75,51.25)(138.75,26.25)
\psline[linewidth=0.75]{<-}(126.25,73.13)(126.25,39.37)
\psline[linewidth=0.75](113.75,85.62)(138.75,60.62)
\psline[linewidth=0.75](23.75,85.63)(73.75,85.62)
\psline[linewidth=0.75](73.75,60.62)(73.75,85.62)
\psline[linewidth=0.75]{<-}(48.75,97.5)(48.75,85.62)
\psline[linewidth=0.75](23.75,60.63)(73.75,60.62)
\psline[linewidth=0.75]{<-}(63.75,60.62)(63.75,0)
\psline[linewidth=0.75]{<-}(33.75,60.63)(33.75,39.37)
\psline[linewidth=0.75](23.75,85.63)(23.75,60.63)
\rput(48.75,72.5){$\gee$}
\psline[linewidth=0.75](3.75,47.49)(25,47.49)
\psline[linewidth=0.75](45,27.5)(23.75,27.5)
\psline[linewidth=0.75](25,47.49)(45,27.5)
\psline[linewidth=0.75](3.75,47.49)(23.75,27.5)
\psline[linewidth=0.75](24.38,10.63)(24.38,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(24.38,10.62){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75]{<-}(35,27.5)(35,21.25)
\psline[linewidth=0.75]{<-}(14.38,36.88)(14.38,20.01)
\psline[linewidth=0.75](35,21.25)(24.38,10.63)
\psline[linewidth=0.75](14.38,20.01)(24.38,10)
\psline[linewidth=0.75]{<-}(145,60.62)(145,0)
\rput(25,36.25){$\parteval$}
\rput[r](143.12,5){\Beliefs}
\rput[l](166.88,5){\Causes}
\rput(0,0){\rput(126.25,55.62){\psframebox[fillcolor=white,fillstyle=solid]{\Beliefs}}}
\rput[r](23.12,4.38){\Beliefs}
\rput[l](65.62,5){\Causes}
\rput[l](35,50){\Beliefs}
\end{pspicture}


==> PICS/kleene-11.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Oct 25 15:24:50 GMT-05:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="13.75" x-max="173.75" y-min="-1.25" y-max="112.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(113.75,94.37);(113.75,94.37);(173.75,94.37);(173.75,94.37)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(113.75,60);(113.75,60);(113.75,35);(113.75,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(173.75,69.37);(173.75,69.37);(173.75,94.37);(173.75,94.37)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(153.75,106.25);(153.75,106.25);(153.75,94.37);(153.75,94.37)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(153.75,112.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165.62,-1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(138.75,69.37);(138.75,69.37);(173.75,69.37);(173.75,69.37)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,69.37);(165,69.37);(165,3.75);(165,3.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(113.75,35);(113.75,35);(138.75,35);(138.75,35)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(151.87,81.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(121.25,41.87)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(98.75,76.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(113.75,60);(113.75,60);(138.75,35);(138.75,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(126.25,81.88);(126.25,81.88);(126.25,48.12);(126.25,48.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(113.75,94.37);(113.75,94.37);(138.75,69.37);(138.75,69.37)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,94.38);(33.75,94.38);(83.75,94.37);(83.75,94.37)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(83.75,69.37);(83.75,69.37);(83.75,94.37);(83.75,94.37)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(58.75,106.25);(58.75,106.25);(58.75,94.37);(58.75,94.37)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(58.75,112.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(74.38,-1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(33.75,69.38);(33.75,69.38);(83.75,69.37);(83.75,69.37)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(73.75,69.37);(73.75,69.37);(73.75,3.75);(73.75,3.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(43.75,69.38);(43.75,69.38);(43.75,48.12);(43.75,48.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,94.38);(33.75,94.38);(33.75,69.38);(33.75,69.38)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(58.75,81.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(13.75,56.24);(13.75,56.24);(35,56.24);(35,56.24)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,36.25);(55,36.25);(33.75,36.25);(33.75,36.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,56.24);(35,56.24);(55,36.25);(55,36.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(13.75,56.24);(13.75,56.24);(33.75,36.25);(33.75,36.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(34.38,14.38);(34.38,14.38);(34.38,3.75);(34.38,3.75)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(35.78,12.96)"
%	 fill-style= "solid"
%	 p2= "(35.78,15.78)"
%	 fill-color= "#330033"
%	 p1= "(32.96,15.78)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,36.25);(45,36.25);(45,25);(45,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(24.38,45);(24.38,45);(24.38,23.76);(24.38,23.76)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,25);(45,25);(34.38,14.38);(34.38,14.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(24.38,23.76);(24.38,23.76);(34.38,13.75);(34.38,13.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,69.37);(145,69.37);(145,3.75);(145,3.75)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(34.38,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<ellipse p3= "(127.81,45.94)"
%	 fill-style= "solid"
%	 p2= "(127.81,49.06)"
%	 p1= "(124.69,49.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(45.31,45.31)"
%	 fill-style= "solid"
%	 p2= "(45.31,48.44)"
%	 p1= "(42.19,48.44)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(173.75,112.5)
\psline[linewidth=0.75](113.75,94.37)(173.75,94.37)
\psline[linewidth=0.75](113.75,60)(113.75,35)
\psline[linewidth=0.75](173.75,69.37)(173.75,94.37)
\psline[linewidth=0.75](153.75,106.25)(153.75,94.37)
\rput(153.75,112.5){$\nameslang$}
\rput(165.62,-1.25){$\inputt$}
\psline[linewidth=0.75](138.75,69.37)(173.75,69.37)
\psline[linewidth=0.75](165,69.37)(165,3.75)
\psline[linewidth=0.75](113.75,35)(138.75,35)
\rput(151.87,81.25){\universal}
\rput(121.25,41.87){\program}
\rput(98.75,76.25){\EQLS}
\psline[linewidth=0.75](113.75,60)(138.75,35)
\psline[linewidth=0.75](126.25,81.88)(126.25,48.12)
\psline[linewidth=0.75](113.75,94.37)(138.75,69.37)
\psline[linewidth=0.75](33.75,94.38)(83.75,94.37)
\psline[linewidth=0.75](83.75,69.37)(83.75,94.37)
\psline[linewidth=0.75](58.75,106.25)(58.75,94.37)
\rput(58.75,112.5){$\nameslang$}
\rput(74.38,-1.25){$\inputt$}
\psline[linewidth=0.75](33.75,69.38)(83.75,69.37)
\psline[linewidth=0.75](73.75,69.37)(73.75,3.75)
\psline[linewidth=0.75](43.75,69.38)(43.75,48.12)
\psline[linewidth=0.75](33.75,94.38)(33.75,69.38)
\rput(58.75,81.25){$\gee$}
\psline[linewidth=0.75](13.75,56.24)(35,56.24)
\psline[linewidth=0.75](55,36.25)(33.75,36.25)
\psline[linewidth=0.75](35,56.24)(55,36.25)
\psline[linewidth=0.75](13.75,56.24)(33.75,36.25)
\psline[linewidth=0.75](34.38,14.38)(34.38,3.75)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(34.37,14.37){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75](45,36.25)(45,25)
\psline[linewidth=0.75](24.38,45)(24.38,23.76)
\psline[linewidth=0.75](45,25)(34.38,14.38)
\psline[linewidth=0.75](24.38,23.76)(34.38,13.75)
\psline[linewidth=0.75](145,69.37)(145,3.75)
\rput(145,-0.62){$\progtype$}
\rput(34.38,-1.25){$\progtype$}
\rput(35,45){$\parteval$}
\rput{0}(126.25,47.5){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(43.75,46.88){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\end{pspicture}


==> PICS/kleene-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Aug 15 21:46:59 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0.12" x-max="343.38" y-min="0" y-max="120" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(98.12,108.12);(98.12,108.12);(158.12,108.12);(158.12,108.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(98.12,73.75);(98.12,73.75);(98.12,48.75);(98.12,48.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(158.12,83.12);(158.12,83.12);(158.12,108.12);(158.12,108.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(138.12,120);(138.12,120);(138.12,108.12);(138.12,108.12)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(123.12,83.12);(123.12,83.12);(158.12,83.12);(158.12,83.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(149.38,83.12);(149.38,83.12);(149.38,2.5);(149.38,2.5)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(98.12,48.75);(98.12,48.75);(123.12,48.75);(123.12,48.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(136.24,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(105.62,55.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(85.62,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(98.12,73.75);(98.12,73.75);(123.12,48.75);(123.12,48.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110.62,95.62);(110.62,95.62);(110.62,61.88);(110.62,61.88)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(98.12,108.12);(98.12,108.12);(123.12,83.12);(123.12,83.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(23.12,108.12);(23.12,108.12);(73.12,108.12);(73.12,108.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(73.12,83.12);(73.12,83.12);(73.12,108.12);(73.12,108.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(48.12,120);(48.12,120);(48.12,108.12);(48.12,108.12)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(23.12,83.12);(23.12,83.12);(73.12,83.12);(73.12,83.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(63.12,83.12);(63.12,83.12);(63.12,1.88);(63.12,1.88)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(33.12,83.12);(33.12,83.12);(33.12,61.87);(33.12,61.87)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(23.12,108.12);(23.12,108.12);(23.12,83.12);(23.12,83.12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(48.12,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(3.12,70);(3.12,70);(24.38,70);(24.38,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(44.38,50);(44.38,50);(23.12,50);(23.12,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(24.38,70);(24.38,70);(44.38,50);(44.38,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(3.12,70);(3.12,70);(23.12,50);(23.12,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(23.75,28.12);(23.75,28.12);(23.75,17.5);(23.75,17.5)"
%	 />
%<ellipse fill-color= "#330033"
%	 p3= "(25.17,26.72)"
%	 p2= "(25.17,29.54)"
%	 fill-style= "solid"
%	 p1= "(22.34,29.54)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(34.38,50);(34.38,50);(34.38,38.75);(34.38,38.75)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(13.74,58.75);(13.74,58.75);(13.74,37.5);(13.74,37.5)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(34.38,38.75);(34.38,38.75);(23.75,28.12);(23.75,28.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(13.74,37.5);(13.74,37.5);(23.75,27.5);(23.75,27.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(129.38,83.12);(129.38,83.12);(129.38,17.5);(129.38,17.5)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(13.12,28.75);(13.12,28.75);(13.12,3.75);(13.12,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(13.12,3.75);(13.12,3.75);(38.12,3.75);(38.12,3.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(20.62,10.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(13.12,28.75);(13.12,28.75);(38.12,3.75);(38.12,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(117.5,29.38);(117.5,29.38);(117.5,4.38);(117.5,4.38)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(117.5,4.38);(117.5,4.38);(142.5,4.38);(142.5,4.38)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(125,11.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(117.5,29.38);(117.5,29.38);(142.5,4.38);(142.5,4.38)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(183.74,107.5);(183.74,107.5);(243.74,107.5);(243.74,107.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(243.74,82.5);(243.74,82.5);(243.74,107.5);(243.74,107.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(223.74,119.38);(223.74,119.38);(223.74,107.5);(223.74,107.5)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(208.74,82.5);(208.74,82.5);(243.74,82.5);(243.74,82.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(235,82.5);(235,82.5);(235,1.88);(235,1.88)"
%	 left-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(221.86,94.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(171.24,89.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(183.74,107.5);(183.74,107.5);(208.74,82.5);(208.74,82.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(205.62,30);(205.62,30);(205.62,19.38);(205.62,19.38)"
%	 />
%<ellipse fill-color= "#330033"
%	 p3= "(207.04,28.59)"
%	 p2= "(207.04,31.41)"
%	 fill-style= "solid"
%	 p1= "(204.21,31.41)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(216.24,82.5);(216.24,82.5);(216.24,40.62);(216.24,40.62)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(195.62,95.62);(195.62,95.62);(195.62,39.38);(195.62,39.38)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(216.24,40.62);(216.24,40.62);(205.62,30);(205.62,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(195.62,39.38);(195.62,39.38);(205.62,29.38);(205.62,29.38)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(195,30.62);(195,30.62);(195,5.62);(195,5.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(195,5.62);(195,5.62);(220,5.62);(220,5.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(202.5,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(195,30.62);(195,30.62);(220,5.62);(220,5.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(290.24,108.12);(290.24,108.12);(343.38,108.12);(343.38,108.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(343.38,83.12);(343.38,83.12);(343.38,108.12);(343.38,108.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(318.38,120);(318.38,120);(318.38,108.12);(318.38,108.12)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(315.24,83.12);(315.24,83.12);(343.38,83.12);(343.38,83.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(333.38,83.12);(333.38,83.12);(333.38,1.88);(333.38,1.88)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(303.38,94.38);(303.38,94.38);(303.38,61.87);(303.38,61.87)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(290.24,108.12);(290.24,108.12);(315.24,83.12);(315.24,83.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(273.38,70);(273.38,70);(294.62,70);(294.62,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(314.62,50);(314.62,50);(293.38,50);(293.38,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(294.62,70);(294.62,70);(314.62,50);(314.62,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(273.38,70);(273.38,70);(293.38,50);(293.38,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(294,28.12);(294,28.12);(294,17.5);(294,17.5)"
%	 />
%<ellipse fill-color= "#330033"
%	 p3= "(295.4,26.72)"
%	 p2= "(295.4,29.54)"
%	 fill-style= "solid"
%	 p1= "(292.6,29.54)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(304.62,50);(304.62,50);(304.62,38.75);(304.62,38.75)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(284,58.75);(284,58.75);(284,37.5);(284,37.5)"
%	 left-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(304.62,38.75);(304.62,38.75);(294,28.12);(294,28.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(284,37.5);(284,37.5);(294,27.5);(294,27.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(283.38,28.75);(283.38,28.75);(283.38,3.75);(283.38,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(283.38,3.75);(283.38,3.75);(308.38,3.75);(308.38,3.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(290.88,10.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(283.38,28.75);(283.38,28.75);(308.38,3.75);(308.38,3.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(325.24,95.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(255.62,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(24.38,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(294,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0.12,99);(0.12,99);(0.12,0);(0.12,0)"
%	 stroke-color= "#ff3333"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0.12,99);(0.12,99);(48.12,51);(48.12,51)"
%	 stroke-color= "#ff3333"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45.88,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\progH
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(48.12,51);(48.12,51);(48.12,0);(48.12,0)"
%	 stroke-color= "#ff3333"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0.12,0);(0.12,0);(48.12,0);(48.12,0)"
%	 stroke-color= "#ff3333"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(270.62,99);(270.62,99);(270.62,0);(270.62,0)"
%	 stroke-color= "#ff3333"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(270.62,99);(270.62,99);(318.62,51);(318.62,51)"
%	 stroke-color= "#ff3333"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(316.38,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\progH
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(318.62,51);(318.62,51);(318.62,0);(318.62,0)"
%	 stroke-color= "#ff3333"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(270.62,0);(270.62,0);(318.62,0);(318.62,0)"
%	 stroke-color= "#ff3333"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(34.38,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Beliefs
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(131.25,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Beliefs
%</text>
%<text fill-color= "#ffffff"
%	 text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(303.75,80)"
%	 text-frame= "rectangle"
%	 text-hor-align= "center-h"
%	 >
%\Beliefs
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(293.75,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Beliefs
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(64.38,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Causes
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150.62,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Causes
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(236.88,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Causes
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(334.38,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Causes
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(205,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Beliefs
%</text>
%<text fill-color= "#ffffff"
%	 text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(110.62,78.75)"
%	 text-frame= "rectangle"
%	 text-hor-align= "center-h"
%	 >
%\Beliefs
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(343.38,120)
\psline[linewidth=0.75](98.12,108.12)(158.12,108.12)
\psline[linewidth=0.75](98.12,73.75)(98.12,48.75)
\psline[linewidth=0.75](158.12,83.12)(158.12,108.12)
\psline[linewidth=0.75]{<-}(138.12,120)(138.12,108.12)
\psline[linewidth=0.75](123.12,83.12)(158.12,83.12)
\psline[linewidth=0.75]{<-}(149.38,83.12)(149.38,2.5)
\psline[linewidth=0.75](98.12,48.75)(123.12,48.75)
\rput(136.24,95){\universal}
\rput(105.62,55.62){\program}
\rput(85.62,90){\EQLS}
\psline[linewidth=0.75](98.12,73.75)(123.12,48.75)
\psline[linewidth=0.75]{<-}(110.62,95.62)(110.62,61.88)
\psline[linewidth=0.75](98.12,108.12)(123.12,83.12)
\psline[linewidth=0.75](23.12,108.12)(73.12,108.12)
\psline[linewidth=0.75](73.12,83.12)(73.12,108.12)
\psline[linewidth=0.75]{<-}(48.12,120)(48.12,108.12)
\psline[linewidth=0.75](23.12,83.12)(73.12,83.12)
\psline[linewidth=0.75]{<-}(63.12,83.12)(63.12,1.88)
\psline[linewidth=0.75]{<-}(33.12,83.12)(33.12,61.87)
\psline[linewidth=0.75](23.12,108.12)(23.12,83.12)
\rput(48.12,95){$\gee$}
\psline[linewidth=0.75](3.12,70)(24.38,70)
\psline[linewidth=0.75](44.38,50)(23.12,50)
\psline[linewidth=0.75](24.38,70)(44.38,50)
\psline[linewidth=0.75](3.12,70)(23.12,50)
\psline[linewidth=0.75](23.75,28.12)(23.75,17.5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(23.76,28.13){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.42,-1.41)}
\psline[linewidth=0.75]{<-}(34.38,50)(34.38,38.75)
\psline[linewidth=0.75]{<-}(13.74,58.75)(13.74,37.5)
\psline[linewidth=0.75](34.38,38.75)(23.75,28.12)
\psline[linewidth=0.75](13.74,37.5)(23.75,27.5)
\psline[linewidth=0.75]{<-}(129.38,83.12)(129.38,17.5)
\psline[linewidth=0.75](13.12,28.75)(13.12,3.75)
\psline[linewidth=0.75](13.12,3.75)(38.12,3.75)
\rput(20.62,10.62){\program}
\psline[linewidth=0.75](13.12,28.75)(38.12,3.75)
\psline[linewidth=0.75](117.5,29.38)(117.5,4.38)
\psline[linewidth=0.75](117.5,4.38)(142.5,4.38)
\rput(125,11.25){\program}
\psline[linewidth=0.75](117.5,29.38)(142.5,4.38)
\psline[linewidth=0.75](183.74,107.5)(243.74,107.5)
\psline[linewidth=0.75](243.74,82.5)(243.74,107.5)
\psline[linewidth=0.75]{<-}(223.74,119.38)(223.74,107.5)
\psline[linewidth=0.75](208.74,82.5)(243.74,82.5)
\psline[linewidth=0.75]{<-}(235,82.5)(235,1.88)
\rput(221.86,94.38){\universal}
\rput(171.24,89.38){\EQLS}
\psline[linewidth=0.75](183.74,107.5)(208.74,82.5)
\psline[linewidth=0.75](205.62,30)(205.62,19.38)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(205.62,30){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.42,-1.41)}
\psline[linewidth=0.75]{<-}(216.24,82.5)(216.24,40.62)
\psline[linewidth=0.75]{<-}(195.62,95.62)(195.62,39.38)
\psline[linewidth=0.75](216.24,40.62)(205.62,30)
\psline[linewidth=0.75](195.62,39.38)(205.62,29.38)
\psline[linewidth=0.75](195,30.62)(195,5.62)
\psline[linewidth=0.75](195,5.62)(220,5.62)
\rput(202.5,12.5){\program}
\psline[linewidth=0.75](195,30.62)(220,5.62)
\psline[linewidth=0.75](290.24,108.12)(343.38,108.12)
\psline[linewidth=0.75](343.38,83.12)(343.38,108.12)
\psline[linewidth=0.75]{<-}(318.38,120)(318.38,108.12)
\psline[linewidth=0.75](315.24,83.12)(343.38,83.12)
\psline[linewidth=0.75]{<-}(333.38,83.12)(333.38,1.88)
\psline[linewidth=0.75]{<-}(303.38,94.38)(303.38,61.87)
\psline[linewidth=0.75](290.24,108.12)(315.24,83.12)
\psline[linewidth=0.75](273.38,70)(294.62,70)
\psline[linewidth=0.75](314.62,50)(293.38,50)
\psline[linewidth=0.75](294.62,70)(314.62,50)
\psline[linewidth=0.75](273.38,70)(293.38,50)
\psline[linewidth=0.75](294,28.12)(294,17.5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(294,28.13){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.4)}
\psline[linewidth=0.75]{<-}(304.62,50)(304.62,38.75)
\psline[linewidth=0.75]{<-}(284,58.75)(284,37.5)
\psline[linewidth=0.75](304.62,38.75)(294,28.12)
\psline[linewidth=0.75](284,37.5)(294,27.5)
\psline[linewidth=0.75](283.38,28.75)(283.38,3.75)
\psline[linewidth=0.75](283.38,3.75)(308.38,3.75)
\rput(290.88,10.62){\program}
\psline[linewidth=0.75](283.38,28.75)(308.38,3.75)
\rput(325.24,95.62){\universal}
\rput(255.62,90){\EQLS}
\rput(24.38,60){$\parteval$}
\rput(294,60){$\parteval$}
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](0.12,99)(0.12,0)
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](0.12,99)(48.12,51)
\rput[r](45.88,25){\progH}
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](48.12,51)(48.12,0)
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](0.12,0)(48.12,0)
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](270.62,99)(270.62,0)
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](270.62,99)(318.62,51)
\rput[r](316.38,25){\progH}
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](318.62,51)(318.62,0)
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](270.62,0)(318.62,0)
\rput[l](34.38,70){\Beliefs}
\rput[l](131.25,30){\Beliefs}
\rput(0,0){\rput(303.75,80){\psframebox[fillcolor=white,fillstyle=solid]{\Beliefs}}}
\rput(293.75,40){\Beliefs}
\rput[l](64.38,6.25){\Causes}
\rput[l](150.62,6.25){\Causes}
\rput[l](236.88,6.25){\Causes}
\rput[l](334.38,6.25){\Causes}
\rput(205,42.5){\Beliefs}
\rput(0,0){\rput(110.62,78.75){\psframebox[fillcolor=white,fillstyle=solid]{\Beliefs}}}
\end{pspicture}


==> PICS/kleene-21.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Oct 25 15:38:19 GMT-05:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="20" x-max="368.75" y-min="0.62" y-max="131.25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(125,113.12);(125,113.12);(185,113.12);(185,113.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,78.75);(125,78.75);(125,53.75);(125,53.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,88.12);(185,88.12);(185,113.12);(185,113.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,125);(165,125);(165,113.12);(165,113.12)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165,131.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(176.25,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,88.12);(150,88.12);(185,88.12);(185,88.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(176.25,88.12);(176.25,88.12);(176.25,7.5);(176.25,7.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,53.75);(125,53.75);(150,53.75);(150,53.75)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(163.12,100)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(132.5,60.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,95)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(125,78.75);(125,78.75);(150,53.75);(150,53.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,100.62);(137.5,100.62);(137.5,66.88);(137.5,66.88)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,113.12);(125,113.12);(150,88.12);(150,88.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,113.12);(45,113.12);(95,113.12);(95,113.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,88.12);(95,88.12);(95,113.12);(95,113.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,125);(70,125);(70,113.12);(70,113.12)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,131.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(45,88.12);(45,88.12);(95,88.12);(95,88.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,88.12);(85,88.12);(85,6.88);(85,6.88)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,88.12);(55,88.12);(55,66.87);(55,66.87)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,113.12);(45,113.12);(45,88.12);(45,88.12)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,75);(25,75);(46.25,75);(46.25,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(66.25,55);(66.25,55);(45,55);(45,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(46.25,75);(46.25,75);(66.25,55);(66.25,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,75);(25,75);(45,55);(45,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45.62,33.12);(45.62,33.12);(45.62,22.5);(45.62,22.5)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(47.04,31.72)"
%	 fill-style= "solid"
%	 p2= "(47.04,34.54)"
%	 fill-color= "#330033"
%	 p1= "(44.22,34.54)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(56.25,55);(56.25,55);(56.25,43.75);(56.25,43.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35.62,63.75);(35.62,63.75);(35.62,42.5);(35.62,42.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(56.25,43.75);(56.25,43.75);(45.62,33.12);(45.62,33.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35.62,42.5);(35.62,42.5);(45.62,32.5);(45.62,32.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(156.25,88.12);(156.25,88.12);(156.25,22.5);(156.25,22.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,33.75);(35,33.75);(35,8.75);(35,8.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,8.75);(35,8.75);(60,8.75);(60,8.75)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(42.5,15.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,33.75);(35,33.75);(60,8.75);(60,8.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(144.38,34.38);(144.38,34.38);(144.38,9.38);(144.38,9.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(144.38,9.38);(144.38,9.38);(169.38,9.38);(169.38,9.38)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(151.88,16.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(144.38,34.38);(144.38,34.38);(169.38,9.38);(169.38,9.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215.62,112.5);(215.62,112.5);(275.62,112.5);(275.62,112.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275.62,87.5);(275.62,87.5);(275.62,112.5);(275.62,112.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255.62,124.38);(255.62,124.38);(255.62,112.5);(255.62,112.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(255.62,130.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(266.88,0.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(240.62,87.5);(240.62,87.5);(275.62,87.5);(275.62,87.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(266.88,87.5);(266.88,87.5);(266.88,6.88);(266.88,6.88)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(253.74,99.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(200.62,94.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(215.62,112.5);(215.62,112.5);(240.62,87.5);(240.62,87.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(237.5,35);(237.5,35);(237.5,24.38);(237.5,24.38)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(238.91,33.59)"
%	 fill-style= "solid"
%	 p2= "(238.91,36.41)"
%	 fill-color= "#330033"
%	 p1= "(236.09,36.41)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(248.12,87.5);(248.12,87.5);(248.12,45.62);(248.12,45.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(227.5,100.62);(227.5,100.62);(227.5,44.38);(227.5,44.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(248.12,45.62);(248.12,45.62);(237.5,35);(237.5,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(227.5,44.38);(227.5,44.38);(237.5,34.38);(237.5,34.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(226.88,35.62);(226.88,35.62);(226.88,10.62);(226.88,10.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(226.88,10.62);(226.88,10.62);(251.88,10.62);(251.88,10.62)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(234.38,17.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(226.88,35.62);(226.88,35.62);(251.88,10.62);(251.88,10.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315.62,113.12);(315.62,113.12);(368.75,113.12);(368.75,113.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(368.75,88.12);(368.75,88.12);(368.75,113.12);(368.75,113.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(343.75,125);(343.75,125);(343.75,113.12);(343.75,113.12)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(343.75,131.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(358.75,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(340.62,88.12);(340.62,88.12);(368.75,88.12);(368.75,88.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(358.75,88.12);(358.75,88.12);(358.75,6.88);(358.75,6.88)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(328.75,99.38);(328.75,99.38);(328.75,66.87);(328.75,66.87)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315.62,113.12);(315.62,113.12);(340.62,88.12);(340.62,88.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(298.75,75);(298.75,75);(320,75);(320,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,55);(340,55);(318.75,55);(318.75,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,75);(320,75);(340,55);(340,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(298.75,75);(298.75,75);(318.75,55);(318.75,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(319.38,33.12);(319.38,33.12);(319.38,22.5);(319.38,22.5)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(320.78,31.72)"
%	 fill-style= "solid"
%	 p2= "(320.78,34.54)"
%	 fill-color= "#330033"
%	 p1= "(317.97,34.54)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,55);(330,55);(330,43.75);(330,43.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(309.38,63.75);(309.38,63.75);(309.38,42.5);(309.38,42.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,43.75);(330,43.75);(319.38,33.12);(319.38,33.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(309.38,42.5);(309.38,42.5);(319.38,32.5);(319.38,32.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(308.75,33.75);(308.75,33.75);(308.75,8.75);(308.75,8.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(308.75,8.75);(308.75,8.75);(333.75,8.75);(333.75,8.75)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(316.25,15.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(308.75,33.75);(308.75,33.75);(333.75,8.75);(333.75,8.75)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(350.62,100.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(291.88,95)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(44.38,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(319.38,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<ellipse p3= "(139.06,64.69)"
%	 fill-style= "solid"
%	 p2= "(139.06,67.81)"
%	 p1= "(135.94,67.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(56.41,64.22)"
%	 fill-style= "solid"
%	 p2= "(56.41,67.04)"
%	 fill-color= "#330033"
%	 p1= "(53.59,67.04)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(157.81,20.94)"
%	 fill-style= "solid"
%	 p2= "(157.81,24.06)"
%	 p1= "(154.69,24.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(239.06,23.44)"
%	 fill-style= "solid"
%	 p2= "(239.06,26.56)"
%	 p1= "(235.94,26.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(330.16,64.84)"
%	 fill-style= "solid"
%	 p2= "(330.16,67.66)"
%	 fill-color= "#330033"
%	 p1= "(327.34,67.66)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(47.18,20.94)"
%	 fill-style= "solid"
%	 p2= "(47.18,24.06)"
%	 p1= "(44.06,24.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(320.94,21.56)"
%	 fill-style= "solid"
%	 p2= "(320.94,24.69)"
%	 p1= "(317.82,24.69)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(295,80);(295,80);(322.5,80);(322.5,80);(322.5,80);(347.5,55);
%	(347.5,55);(347.5,55);(347.5,5);(347.5,5);(347.5,5);(295,5);
%	(295,5);(295,5);(295,5);(295,5);(295,5);(295,80)"
%	 stroke-color= "#cc0033"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(335,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Gee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,80);(20,80);(47.5,80);(47.5,80);(47.5,80);(72.5,55);
%	(72.5,55);(72.5,55);(72.5,5);(72.5,5);(72.5,5);(20,5);
%	(20,5);(20,5);(20,5);(20,5);(20,5);(20,80)"
%	 stroke-color= "#cc0033"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Gee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(368.75,131.25)
\psline[linewidth=0.75](125,113.12)(185,113.12)
\psline[linewidth=0.75](125,78.75)(125,53.75)
\psline[linewidth=0.75](185,88.12)(185,113.12)
\psline[linewidth=0.75](165,125)(165,113.12)
\rput(165,131.25){$\nameslang$}
\rput(176.25,1.25){$\inputt$}
\psline[linewidth=0.75](150,88.12)(185,88.12)
\psline[linewidth=0.75](176.25,88.12)(176.25,7.5)
\psline[linewidth=0.75](125,53.75)(150,53.75)
\rput(163.12,100){\universal}
\rput(132.5,60.62){\program}
\rput(110,95){\EQLS}
\psline[linewidth=0.75](125,78.75)(150,53.75)
\psline[linewidth=0.75](137.5,100.62)(137.5,66.88)
\psline[linewidth=0.75](125,113.12)(150,88.12)
\psline[linewidth=0.75](45,113.12)(95,113.12)
\psline[linewidth=0.75](95,88.12)(95,113.12)
\psline[linewidth=0.75](70,125)(70,113.12)
\rput(70,131.25){$\nameslang$}
\rput(85,1.25){$\inputt$}
\psline[linewidth=0.75](45,88.12)(95,88.12)
\psline[linewidth=0.75](85,88.12)(85,6.88)
\psline[linewidth=0.75](55,88.12)(55,66.87)
\psline[linewidth=0.75](45,113.12)(45,88.12)
\rput(70,100){$\gee$}
\psline[linewidth=0.75](25,75)(46.25,75)
\psline[linewidth=0.75](66.25,55)(45,55)
\psline[linewidth=0.75](46.25,75)(66.25,55)
\psline[linewidth=0.75](25,75)(45,55)
\psline[linewidth=0.75](45.62,33.12)(45.62,22.5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(45.63,33.13){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75](56.25,55)(56.25,43.75)
\psline[linewidth=0.75](35.62,63.75)(35.62,42.5)
\psline[linewidth=0.75](56.25,43.75)(45.62,33.12)
\psline[linewidth=0.75](35.62,42.5)(45.62,32.5)
\psline[linewidth=0.75](156.25,88.12)(156.25,22.5)
\psline[linewidth=0.75](35,33.75)(35,8.75)
\psline[linewidth=0.75](35,8.75)(60,8.75)
\rput(42.5,15.62){\program}
\psline[linewidth=0.75](35,33.75)(60,8.75)
\psline[linewidth=0.75](144.38,34.38)(144.38,9.38)
\psline[linewidth=0.75](144.38,9.38)(169.38,9.38)
\rput(151.88,16.25){\program}
\psline[linewidth=0.75](144.38,34.38)(169.38,9.38)
\psline[linewidth=0.75](215.62,112.5)(275.62,112.5)
\psline[linewidth=0.75](275.62,87.5)(275.62,112.5)
\psline[linewidth=0.75](255.62,124.38)(255.62,112.5)
\rput(255.62,130.62){$\nameslang$}
\rput(266.88,0.62){$\inputt$}
\psline[linewidth=0.75](240.62,87.5)(275.62,87.5)
\psline[linewidth=0.75](266.88,87.5)(266.88,6.88)
\rput(253.74,99.38){\universal}
\rput(200.62,94.38){\EQLS}
\psline[linewidth=0.75](215.62,112.5)(240.62,87.5)
\psline[linewidth=0.75](237.5,35)(237.5,24.38)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(237.5,35){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75](248.12,87.5)(248.12,45.62)
\psline[linewidth=0.75](227.5,100.62)(227.5,44.38)
\psline[linewidth=0.75](248.12,45.62)(237.5,35)
\psline[linewidth=0.75](227.5,44.38)(237.5,34.38)
\psline[linewidth=0.75](226.88,35.62)(226.88,10.62)
\psline[linewidth=0.75](226.88,10.62)(251.88,10.62)
\rput(234.38,17.5){\program}
\psline[linewidth=0.75](226.88,35.62)(251.88,10.62)
\psline[linewidth=0.75](315.62,113.12)(368.75,113.12)
\psline[linewidth=0.75](368.75,88.12)(368.75,113.12)
\psline[linewidth=0.75](343.75,125)(343.75,113.12)
\rput(343.75,131.25){$\nameslang$}
\rput(358.75,1.25){$\inputt$}
\psline[linewidth=0.75](340.62,88.12)(368.75,88.12)
\psline[linewidth=0.75](358.75,88.12)(358.75,6.88)
\psline[linewidth=0.75](328.75,99.38)(328.75,66.87)
\psline[linewidth=0.75](315.62,113.12)(340.62,88.12)
\psline[linewidth=0.75](298.75,75)(320,75)
\psline[linewidth=0.75](340,55)(318.75,55)
\psline[linewidth=0.75](320,75)(340,55)
\psline[linewidth=0.75](298.75,75)(318.75,55)
\psline[linewidth=0.75](319.38,33.12)(319.38,22.5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(319.38,33.13){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.4)}
\psline[linewidth=0.75](330,55)(330,43.75)
\psline[linewidth=0.75](309.38,63.75)(309.38,42.5)
\psline[linewidth=0.75](330,43.75)(319.38,33.12)
\psline[linewidth=0.75](309.38,42.5)(319.38,32.5)
\psline[linewidth=0.75](308.75,33.75)(308.75,8.75)
\psline[linewidth=0.75](308.75,8.75)(333.75,8.75)
\rput(316.25,15.62){\program}
\psline[linewidth=0.75](308.75,33.75)(333.75,8.75)
\rput(350.62,100.62){\universal}
\rput(291.88,95){\EQLS}
\rput(44.38,65){$\parteval$}
\rput(319.38,65){$\parteval$}
\rput{0}(137.5,66.25){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(55,65.63){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\rput{0}(156.25,22.5){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(237.5,25){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(328.75,66.25){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\rput{0}(45.62,22.5){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{90}(319.38,23.12){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\newrgbcolor{userLineColour}{0.8 0 0.2}
\pscustom[linewidth=0.45,linecolor=userLineColour]{\psline(295,80)(322.5,80)
\psline(322.5,80)(347.5,55)
\psline(347.5,55)(347.5,5)
\psline(347.5,5)(295,5)
\psbezier(295,5)(295,5)(295,5)
\psline(295,5)(295,80)
\closepath}
\rput(335,25){$\Gee$}
\newrgbcolor{userLineColour}{0.8 0 0.2}
\pscustom[linewidth=0.45,linecolor=userLineColour]{\psline(20,80)(47.5,80)
\psline(47.5,80)(72.5,55)
\psline(72.5,55)(72.5,5)
\psline(72.5,5)(20,5)
\psbezier(20,5)(20,5)(20,5)
\psline(20,5)(20,80)
\closepath}
\rput(60,25){$\Gee$}
\end{pspicture}


==> PICS/kleene.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Aug 15 13:17:31 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="140" y-min="-0.62" y-max="76.88" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(90,65);(90,65);(140,65);(140,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(90,30.62);(90,30.62);(90,5.62);(90,5.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(140,40);(140,40);(140,65);(140,65)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(130,76.88);(130,76.88);(130,65);(130,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,40);(115,40);(140,40);(140,40)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(130,40);(130,40);(130,-0.62);(130,-0.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(90,5.62);(90,5.62);(115,5.62);(115,5.62)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(122.5,52.5)"
%	 stroke-width= "0.75"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(98.75,12.5)"
%	 stroke-width= "0.75"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(75,51.25)"
%	 stroke-width= "0.75"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(90,30.62);(90,30.62);(115,5.62);(115,5.62)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(102.5,52.5);(102.5,52.5);(102.5,18.75);(102.5,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(90,65);(90,65);(115,40);(115,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,65);(5,65);(55,65);(55,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(2.5,30.62);(2.5,30.62);(2.5,5.62);(2.5,5.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(55,40);(55,40);(55,65);(55,65)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,76.88);(30,76.88);(30,65);(30,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,40);(5,40);(55,40);(55,40)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(45,40);(45,40);(45,-0.62);(45,-0.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(2.5,5.62);(2.5,5.62);(27.5,5.62);(27.5,5.62)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(11.25,12.5)"
%	 stroke-width= "0.75"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(2.5,30.62);(2.5,30.62);(27.5,5.62);(27.5,5.62)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,40);(15,40);(15,18.75);(15,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,65);(5,65);(5,40);(5,40)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(46.25,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Causes
%</text>
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 fill-color= "#ffffff"
%	 anchor-point= "(16.25,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Beliefs
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(131.25,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Causes
%</text>
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 fill-color= "#ffffff"
%	 anchor-point= "(103.75,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Beliefs
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(28.75,70.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\Effects
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(128.75,70.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\Effects
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(140,76.88)
\psline[linewidth=0.75](90,65)(140,65)
\psline[linewidth=0.75](90,30.62)(90,5.62)
\psline[linewidth=0.75](140,40)(140,65)
\psline[linewidth=0.75]{<-}(130,76.88)(130,65)
\psline[linewidth=0.75](115,40)(140,40)
\psline[linewidth=0.75]{<-}(130,40)(130,-0.62)
\psline[linewidth=0.75](90,5.62)(115,5.62)
\rput(122.5,52.5){\universal}
\rput(98.75,12.5){\program}
\rput(75,51.25){\EQLS}
\psline[linewidth=0.75](90,30.62)(115,5.62)
\psline[linewidth=0.75]{<-}(102.5,52.5)(102.5,18.75)
\psline[linewidth=0.75](90,65)(115,40)
\psline[linewidth=0.75](5,65)(55,65)
\psline[linewidth=0.75](2.5,30.62)(2.5,5.62)
\psline[linewidth=0.75](55,40)(55,65)
\psline[linewidth=0.75]{<-}(30,76.88)(30,65)
\psline[linewidth=0.75](5,40)(55,40)
\psline[linewidth=0.75]{<-}(45,40)(45,-0.62)
\psline[linewidth=0.75](2.5,5.62)(27.5,5.62)
\rput(11.25,12.5){\program}
\psline[linewidth=0.75](2.5,30.62)(27.5,5.62)
\psline[linewidth=0.75]{<-}(15,40)(15,18.75)
\psline[linewidth=0.75](5,65)(5,40)
\rput(30,52.5){$\gee$}
\rput[l](46.25,3.75){\Causes}
\rput[l](16.25,30){\Beliefs}
\rput[l](131.25,3.75){\Causes}
\rput[l](103.75,30){\Beliefs}
\rput[r](28.75,70.62){\Effects}
\rput[r](128.75,70.62){\Effects}
\end{pspicture}

